On Budgeted Influence Maximization in Social Networks

Given a budget and arbitrary cost for selecting each node, the budgeted influence maximization (BIM) problem concerns selecting a set of seed nodes to disseminate some information that maximizes the total number of nodes influenced (termed as influence spread) in social networks at a total cost no more than the budget. Our proposed seed selection algorithm for the BIM problem guarantees an approximation ratio of (1 - 1/sqrt(e)). The seed selection algorithm needs to calculate the influence spread of candidate seed sets, which is known to be #P-complex. Identifying the linkage between the computation of marginal probabilities in Bayesian networks and the influence spread, we devise efficient heuristic algorithms for the latter problem. Experiments using both large-scale social networks and synthetically generated networks demonstrate superior performance of the proposed algorithm with moderate computation costs. Moreover, synthetic datasets allow us to vary the network parameters and gain important insights on the impact of graph structures on the performance of different algorithms.

==> icdcs12 arxiv/Commands.tex <==
%!TEX root = MultiAgentBandit.tex
%\usepackage[textwidth=18\marginparwidth]{todonotes}
%\usepackage{pdfsync}

%% For citations
%\usepackage{natbib}
%%\bibliographystyle{apalike}
%
%\if0
%\newcommand{\citep}[1]{\cite{#1}}
%\newcommand{\citet}[1]{\cite{#1}}
%\newcommand{\citealt}[1]{\cite{#1}}
%\newcommand{\iftextcite}[1]{}
%
%\newcommand{\npcite}[1]{\cite{#1}}
%\newcommand{\yrcite}[1]{\cite{#1}}
%\fi

% this package is used for making lists inline in a paragraph.
% to use, do: \begin{inparaenum} \item ... \item ... \end{inparaenum}
\usepackage{paralist}

%\usepackage[vlined,algonl,boxed]{algorithm2e}
\usepackage[ruled,vlined]{algorithm2e}
%\usepackage{algpseudocode}

%\usepackage{amsthm}

\usepackage{amssymb}
%\usepackage[dvips]{graphics}
\usepackage{amsmath} % Learn about the AMS package, again very useful!
\usepackage{verbatim}
\usepackage{array}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{stmaryrd}
%\usepackage{color}
%\usepackage{algorithm,algorithmic}
\usepackage{dsfont}
\usepackage{subfig}
\usepackage{soul}

\usepackage{framed}
\usepackage[dvipsnames]{color}
\definecolor{shadecolor}{gray}{0.85}

%\usepackage{small-headings}

\newif\iflong % Sometimes we want to keep two versions; a short and a long one -- this is useful for that..
\longfalse
%\longtrue

\newif\ifcomm
%\commfalse
\commtrue

% THEOREMS -------------------------------------------------------
\newtheorem{thm}{Theorem}
\newtheorem{cor}{Corollary}
\newtheorem{lem}{Lemma}
\newtheorem{prop}{Proposition}
\newtheorem{conj}[thm]{Conjecture}
\newtheorem{proofthm}{Proof of Theorem 2}
\newtheorem{defn}{Definition}
\newtheorem{rem}{Remark}
\newtheorem{ex}{Example}
\newtheorem{remark}{Remark}

% MATH -----------------------------------------------------------
\newcommand{\norm}[1]{\left\Vert#1\right\Vert}
\newcommand{\abs}[1]{\left\vert#1\right\vert}
\newcommand{\set}[1]{\left\{#1\right\}}
\newcommand{\reals}{\mathbb{R}}
\newcommand{\rationals}{\mathbb{Q}}
\newcommand{\integers}{\mathbb{Z}}
\newcommand{\naturals}{\mathbb{N}}
\newcommand{\eps}{\varepsilon}
\newcommand{\To}{\longrightarrow}
\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}
\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\partialderiv}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\ds}{\displaystyle}
\newcommand{\argmin}{\arg\min}
\newcommand{\argmax}{\arg\max}
\newcommand{\sq}{\hbox{\rlap{$\sqcap$}$\sqcup$}}
\DeclareMathOperator{\signmax}{signmax}

\newcommand{\smallnorm}[1]{\|#1\|}
\newcommand{\supnorm}[1]{\norm{#1}_\infty}
\newcommand{\cset}[2]{\left\{\,#1\,:\,#2\,\right\}}
\renewcommand{\natural}{\mathbb N}                   % Natural numbers
\newcommand{\Real}{\mathbb R}                        % Real numbers
\newcommand{\real}{\mathbb R}                        % again..
\newcommand{\R}{{\mathbb{R}}}                        % again..

\newcommand{\Prob}[1]{{\mathbb P}\left(#1\right)}    % Probabilities; example: \Prob{X>\eps}<1-\delta
\renewcommand{\P}{{\mathbb P}}                         % Probabilities when we want to control the parenthesis
\newcommand{\EE}[1]{{\mathbb E}\left[#1\right]}      % Expectations
\newcommand{\E}{{\mathbb E}}                         % Expectations  when we want to control the parenthesis
\newcommand{\Var}[1]{{\mathrm{Var}}\left[#1\right]}  % Variances
%\newcommand{\one}{\mathbb I}
\newcommand{\one}[1]{{\mathbb I}_{\{#1\}}}           % Characteristic function

\newcommand{\scons}{$s$-constraint}
\newcommand{\ucons}{$u$-constraint}
\newcommand{\sort}{\begin{verbatim} sort \end{verbatim}}

\newcommand{\mec}{{\sc mec}}
\newcommand{\tsat}{{\sc 3sat}}
\newcommand{\montsat}{{\sc monotone-3sat}}
\newcommand{\mcgbc}{{\sc mc-gbc}}
\newcommand{\greedy}{{\sc Greedy}}
\newcommand{\probrand}{{\sc ProbRand}}
\newcommand{\piperand}{{\sc PipeRand}}
\newcommand{\pbar}{\overline{p}}
\newcommand{\gammahat}{\hat{\gamma}}

\newenvironment{proof-sketch}{{\noindent\em Proof Sketch.}\hspace*{0.3em}}{\qed\medskip}
%\newenvironment{proof}{{\bf Proof.}}{\hfill\rule{2mm}{2mm}\\}
\newenvironment{proof-of}[1]{{\noindent\em Proof of #1.}\hspace*{0.3em}}{\qed\medskip}



\newcounter{assumption}%[section]
\newcommand{\theassumptionletter}{A}
\renewcommand{\theassumption}{\theassumptionletter\arabic{assumption}}

\newenvironment{ass}[1][]{\begin{trivlist}\item[] \refstepcounter{assumption}%
 {\bf Assumption\ \theassumption\ #1} }{%\par\nobreak\noindent\sl\ignorespaces}{%
 \ifvmode\smallskip\fi\end{trivlist}}
\newcommand{\aref}[1]{(\ref{#1})}



% Keep whatever you need from here

\newcommand{\MB}{\mathcal{B}}
\newcommand{\MA}{\mathcal{A}}
\newcommand{\MG}{\mathcal{G}}
\newcommand{\MS}{\mathcal{S}}
\newcommand{\MF}{\mathcal{F}}
\newcommand{\MC}{\mathcal{C}}
\newcommand{\MRR}{\mathcal{R}}
\newcommand{\MD}{\mathcal{D}}
\newcommand{\MH}{\mathcal{H}}
\newcommand{\MP}{\mathcal{P}}
\newcommand{\MU}{\mathcal{U}}
\newcommand{\MO}{\mathcal{O}}
\newcommand{\MX}{\mathcal{X}}
\newcommand{\MR}{\mathcal{R}}
\newcommand{\MQ}{\mathcal{Q}}
\newcommand{\MT}{\mathcal{T}}
\newcommand{\GG}{\mathcal{G}}
\newcommand{\hZ}{\hat{Z}}
\newcommand{\hF}{\hat{F}}
\newcommand{\hL}{\hat{L}}
\newcommand{\tL}{\tilde{L}}

\newcommand{\MI}{{\bf I}} %\mathbb{I}}


\newcommand{\ep}{\varepsilon}                        % Shorthand for nice epsilon
\newcommand{\de}{\delta}                             % Shorthand for delta
\newcommand{\ra}{\rightarrow}
\newcommand{\diag}{\mathop{\rm diag}}
\newcommand{\inlinemin}{\wedge}
\newcommand{\inlinemax}{\vee}

\newcommand{\ip}[2]{\langle #1,#2 \rangle}
\newcommand{\eqdef}{\stackrel{\mbox{\rm\tiny def}}{=}}
\newcommand{\aP}{{\cal P}}

% Shorthands I use for math environments
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\beqa}{\begin{eqnarray}}
\newcommand{\eeqa}{\end{eqnarray}}
\newcommand{\beqan}{\begin{eqnarray*}}
\newcommand{\eeqan}{\end{eqnarray*}}
\newcommand{\ben}{\begin{eqnarray*}}
\newcommand{\een}{\end{eqnarray*}}

\newcommand{\RA}{$\Rightarrow$}
\ifcomm
   \newcommand\comm[1]{\textcolor{blue}{ #1}}
\else
   \newcommand\comm[1]{}
   \renewcommand{\todo}[1]{}
\fi
\newcommand{\remove}[1]{\textcolor{blue}{\sout{#1}}}
\newcommand{\tO}{\tilde{O}}

% Boldfaced lowercase greek letters as described at
% http://www.rpi.edu/dept/acs/rpinfo/common/Computing/Consulting/Software/LaTeX/Hints/Greek_Chars.html
\def\bmath#1{\mbox{\boldmath$#1$}}
% http://www.ctan.org/tex-archive/info/symbols/comprehensive/symbols-a4.pdf page 68
\newcommand\independent{\protect\mathpalette{\protect\independenT}{\perp}}
\def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern2mu{#1#2}}}

\newcommand{\bm}{\boldmath}
%\newcommand{\beq}{\begin{equation}}
%\newcommand{\eeq}{\end{equation}}
\newcommand{\Nbar}{\bar N}
\newcommand{\lra}{\longrightarrow}
\newcommand{\lla}{\longleftarrow}
\newcommand{\mc}{\multicolumn}
%\newcommand{\qed}{{\hfill$\Box$}}
\newcommand{\C}{\mbox{\bm $C$}}
\newcommand{\Cs}{\mbox{\scriptsize\bm $C$}}
\newcommand{\cc}{\mbox{\bm $c$}}
\newcommand{\bb}{\mbox{\bm $b$}}
\newcommand{\m}{\mbox{\bm $m$}}
\newcommand{\PP}{\mbox{\bm $P$}}
\newcommand{\uu}{\mbox{\bm $u$}}
\newcommand{\Gg}{\mbox{\bm $g$}}
\newcommand{\ccc}{{\bf c}}
\newcommand{\sss}{\mbox{\bm $s$}}
\newcommand{\ttt}{\mbox{$\mathbf{t}$}}
\newcommand{\xx}{\mbox{$\mathbf{x}$}}
\newcommand{\xxx}{{\bm x}}
\newcommand{\rr}{\mbox{\bm $r$}}
\newcommand{\Z}{\mbox{\bm $Z$}}
\newcommand{\0}{{\bf 0}}
\newcommand{\N}{{\cal N}}
\newcommand{\zero}{\mbox{\bm  $0$}}
\newcommand{\vv}{\mbox{\bm $v$}}
\newcommand{\vvb}{\mbox{\scriptsize\bm $v$}}
\newcommand{\yy}{\mbox{$\mathbf y$}}
\newcommand{\G}{\mbox{\bm $G$}}
\newcommand{\I}{\mbox{\bm $I$}}
\newcommand{\A}{\mbox{\bm $A$}}
\newcommand{\B}{\mbox{\bm $B$}}
\newcommand{\T}{\mbox{\bm $T$}}
\newcommand{\X}{\mbox{\bm $X$}}
\newcommand{\bydef}{{\buildrel{\triangle}\over =}}
\newcommand{\tht}{\theta}
\newcommand{\Zhat}{{\hat Z}}
\newcommand{\yhat}{{\hat y}}
\newcommand{\dbar}{{\bar d}}
\newcommand{\cund}{{\underline c}}
\newcommand{\Nhat}{{\hat N}}
\newcommand{\mubar}{{\bar\mu}}
\newcommand{\sigmahat}{{\hat \sigma}}
\newcommand{\sigmabar}{{\bar \sigma}}
\newcommand{\si}{{\sigma}}
\newcommand{\rhohat}{{\hat \rho}}
\newcommand{\thetahat}{{\hat \theta}}
\newcommand{\xb}  {{\mbox{\boldmath $x$}}}
\newcommand{\vb}  {{\mbox{\boldmath $v$}}}
\newcommand{\mem}[1]{\label{eq:#1}}
\newcommand{\rec}[1]{(\ref{eq:#1})}
\newcommand{\nono}{\nonumber}
\newcommand{\scc}{{\cal S}}
\newcommand{\yc}{{\cal C}}
\newcommand{\Cb}  {{\mbox{\boldmath $C$}}}

